Maybe there's no such thing as a random sequence

An infinite binary sequence is deemed to be random if it has all definable properties that hold almost surely for the usual probability measure on the set of infinite binary sequences. There are only countably many such properties, so it would seem that the set of random sequences should have full measure. But in fact there might be no random sequences, because for all we know, there might be no undefinable sets.

==> random_dot_bib <==
@book {cohen:continuum,
    AUTHOR = {Cohen, Paul J.},
     TITLE = {Set theory and the continuum hypothesis},
 PUBLISHER = {W. A. Benjamin},
      YEAR = {1966}
}

@incollection {robinson:64,
    AUTHOR = {Robinson, Abraham},
     TITLE = {Formalism {$64$}},
 BOOKTITLE = {Logic, {M}ethodology and {P}hilos. {S}ci. ({P}roc. 1964
              {I}nternat. {C}ongr.)},
     PAGES = {228--246},
 PUBLISHER = {North-Holland},
      YEAR = {1965}
}

@incollection {cohen:comments,
    AUTHOR = {Cohen, Paul J.},
     TITLE = {Comments on the foundations of set theory},
 BOOKTITLE = {Axiomatic {S}et {T}heory ({P}roc. {S}ympos. {P}ure {M}ath.,
              {V}ol. {XIII}, {P}art {I}, {U}niv. {C}alifornia, {L}os
              {A}ngeles, {C}alif., 1967)},
     PAGES = {9--15},
 PUBLISHER = {Amer. Math. Soc.},
   ADDRESS = {Providence, R.I.},
      YEAR = {1971},
   MRCLASS = {00.50 (02.00)},
  MRNUMBER = {0277332 (43 \#3067)},
MRREVIEWER = {J. W. Robbin},
}

@incollection {tarski:definable,
    AUTHOR = {Tarski, Alfred},
TITLE={On definable sets of real numbers},
     BOOKTITLE = {Logic, {S}emantics, {M}etamathematics. {P}apers from 1923 to 1938},
      NOTE = {Translated by J. H. Woodger},
 PUBLISHER = {Oxford at the Clarendon Press},
      YEAR = {1956},
     PAGES = {110--142}
}

@article{tarski:definissable,
AUTHOR={Tarski, Alfred},
TITLE={Sur les ensembles d\'efinissables de nombers r\'eels},
JOURNAL={Fundamenta Mathematicae},
PAGES={210--239},
YEAR={1931},
VOLUME={17}
}

@article {downeyetal:calibrating,
    AUTHOR = {Downey, Rod and Hirschfeldt, Denis R. and Nies, Andr{\'e} and
              Terwijn, Sebastiaan A.},
     TITLE = {Calibrating randomness},
   JOURNAL = {Bull. Symbolic Logic},
  FJOURNAL = {Bulletin of Symbolic Logic},
    VOLUME = {12},
      YEAR = {2006},
    NUMBER = {3},
     PAGES = {411--491},
      ISSN = {1079-8986},
   MRCLASS = {03D80 (60A05 68Q30)},
  MRNUMBER = {2248591 (2007j:03055)},
MRREVIEWER = {Jan Reimann},
       URL = {http://projecteuclid.org/getRecord?id=euclid.bsl/1154698741},
}

@book{downeyhirschfeldt:algorithmic,
    AUTHOR = {Downey, Rod and Hirschfeldt, Denis R.},
     TITLE = {Algorithmic Randomness and Complexity},
PUBLISHER={Springer},
      YEAR = {2010}
}

@misc{hamkinsetal:pointwise,
title = {Pointwise definable models of set theory},
author = {Hamkins, Joel David and Linetsky, David and Reitz, Jonas},
year="2010",
howpublished= {preprint}}

@book {nies:randomness,
    AUTHOR = {Nies, Andr{\'e}},
     TITLE = {Computability and randomness},
    SERIES = {Oxford Logic Guides},
    VOLUME = {51},
 PUBLISHER = {Oxford University Press},
   ADDRESS = {Oxford},
      YEAR = {2009},
     PAGES = {xvi+433},
      ISBN = {978-0-19-923076-1},
   MRCLASS = {03-02 (03D25 03D28 03D32 03D55 91A60)},
  MRNUMBER = {2548883},
       DOI = {10.1093/acprof:oso/9780199230761.001.0001},
       URL = {http://dx.doi.org/10.1093/acprof:oso/9780199230761.001.0001},
}

